Automated Adversarial Discovery for Safety Classifiers

Safety classifiers are critical in mitigating toxicity on online forums such as social media and in chatbots. Still, they continue to be vulnerable to emergent, and often innumerable, adversarial attacks. Traditional automated adversarial data generation methods, however, tend to produce attacks that are not diverse, but variations of previously observed harm types. We formalize the task of automated adversarial discovery for safety classifiers - to find new attacks along previously unseen harm dimensions that expose new weaknesses in the classifier. We measure progress on this task along two key axes (1) adversarial success: does the attack fool the classifier? and (2) dimensional diversity: does the attack represent a previously unseen harm type? Our evaluation of existing attack generation methods on the CivilComments toxicity task reveals their limitations: Word perturbation attacks fail to fool classifiers, while prompt-based LLM attacks have more adversarial success, but lack dimensional diversity. Even our best-performing prompt-based method finds new successful attacks on unseen harm dimensions of attacks only 5\% of the time. Automatically finding new harmful dimensions of attack is crucial and there is substantial headroom for future research on our new task.

==> tables/identity_attack_results.tex <==
\begin{table*}[!tbh]
\centering
\begin{tabular}{|l|r|r|r|}
\hline
Method & Adversarial Success ($\uparrow$) & Identity Attack \% ($\uparrow$) & Both ($\uparrow$) \\ \hline
EDA & 2.0 $\pm$ 0.00  & 12.0 $\pm$ 0.00 & 0.0 $\pm$ 0.00 \\
WordNet & 6.0 $\pm$ 0.00 & 10.0 $\pm$ 0.00 & 0.0 $\pm$ 0.00 \\
CLARE & 8.0 $\pm$ 0.00 & 16 $\pm$ 0.00 & 0.0 $\pm$ 0.00 \\ \hline
Polyjuice & 43.6 $\pm$ 2.15 & 7.4 $\pm$ 1.56 & 2.8 $\pm$ 1.33 \\
Rewrite & 48.2 $\pm$ 6.03 & 7.4 $\pm$ 3.16 & 2.4 $\pm$ 2.15 \\
Self-Refine & \textbf{57.2 $\pm$ 5.74} & 3.8 $\pm$ 2.75 & 0 $\pm$ 0 \\ \hline
Discover-Adapt (In-Seed) & 38.2 $\pm$ 5.83 & 13.4 $\pm$ 4.90 & 4.4 $\pm$ 2.15 \\
Discover-Adapt (Const 5) & 24 $\pm$ 10.73 & 16 $\pm$ 4.29 & 1.4 $\pm$ 1.56 \\
Discover-Adapt (Const 25) & 30 $\pm$ 6.81 & 19.8 $\pm$ 5.02 & 4.4 $\pm$ 1.50 \\
Discover-Adapt (Const sampled 5) & 21.6 $\pm$ 6.05 & \textbf{26 $\pm$ 4.73} & \textbf{5 $\pm$ 3.82} \\ \hline
\end{tabular}
\caption{We use a variety of metrics to show that our framework of generating adversarial data is better than existing method. The `Both' metric represents the percentage of generated data point that contain identity attacks as well as adversarial for the classifier. We generate data from each method using only a seed set of 25 examples that do not contain identity attacks (held-out dimension). Since the amount of data generated by different methods varies, we report the mean and standard deviation for each method on a sample size of 50 data points bootstrapped for 10 iterations. Here, we treat identity attack as the held-out dimension.}
\label{tab:identity-attack-results}
\end{table*}

==> tables/obscene_results.tex <==
% \begin{table*}[!tbh]
% \centering
% \begin{tabular}{|l|r|r|r|}
% \hline
% Method & Adversarial Success ($\uparrow$) & Held-out Dimension \% ($\uparrow$) & Both ($\uparrow$) \\ \hline
% EDA & 14.0 $\pm$ 0.00  & 30.0 $\pm$ 0.00 & 0.0 $\pm$ 0.00 \\
% WordNet & 18.0 $\pm$ 0.00 & \textbf{34.0 $\pm$ 0.00} & 2.0 $\pm$ 0.00 \\
% CLARE & 22.0 $\pm$ 0.00 & 28 $\pm$ 0.00 & 0.0 $\pm$ 0.00 \\ \hline
% Polyjuice & 47.8 $\pm$ 4.24 & 13.2 $\pm$ 2.44 & 0.8 $\pm$ 0.98 \\
% Rewrite & 48.8 $\pm$ 5.74 & 9.2 $\pm$ 3.12 & 0.0 $\pm$ 0.00 \\
% Self-Refine & \textbf{55.6 $\pm$ 4.63} & 5.8 $\pm$ 2.6 & 0 $\pm$ 0 \\ \hline
% Discover-Adapt (In-Seed) & 42.8 $\pm$ 8.73 & 14 $\pm$ 3.63 & 0.2 $\pm$ 0.6 \\
% Discover-Adapt (Const 5) & 32.4 $\pm$ 5.43 & 17.6 $\pm$ 5.71& \textbf{1.2 $\pm$ 0.98} \\
% Discover-Adapt (Const 25) & 32.2 $\pm$ 4.6 & 23.2 $\pm$ 5.00 & 1.2 $\pm$ 1.33 \\
% Discover-Adapt (Const sampled 5) & 26 $\pm$ 5.14 & 25.2 $\pm$ 1.92 & 1.0 $\pm$ 1.00 \\ \hline
% \end{tabular}
% \caption{When we treat obscene as the held-out dimension, our approach generates more adversarial examples from that dimension. Since the amount of data generated by different methods varies, we report the mean and standard deviation for each method on a sample size of 50 data points bootstrapped for 10 iterations.}
% \label{tab:obscene-results}
% \end{table*}

\begin{table*}[!tbh]
\centering
\begin{tabular}{|l|r|r|r|}
\hline
Method & Adversarial Success ($\uparrow$) & Obscene \% ($\uparrow$) & Both ($\uparrow$) \\ \hline
WordNet & 18.0 $\pm$ 0.00 & \textbf{34.0 $\pm$ 0.00} & \textbf{2.0 $\pm$ 0.00} \\ \hline
Self-Refine & \textbf{55.6 $\pm$ 4.63} & 5.8 $\pm$ 2.6 & 0 $\pm$ 0 \\ \hline
Discover-Adapt (Const 5) & 32.4 $\pm$ 5.43 & 17.6 $\pm$ 5.71& 1.2 $\pm$ 0.98 \\ \hline
\end{tabular}
\caption{When we treat obscene as the held-out dimension, our approach generates more adversarial examples from that dimension. The `Both' metric represents the percentage of generated data point that contain obscenities as well as adversarial for the classifier. Since the amount of data generated by different methods varies, we report the mean and standard deviation for each method on a sample size of 50 data points bootstrapped for 10 iterations. We only report results of the strongest performing methods of each type.}
\label{tab:obscene-results}
\end{table*}

==> tables/threat_results.tex <==
\begin{table*}[!tbh]
\centering
\begin{tabular}{|l|r|r|r|}
\hline
Method & Adversarial Success ($\uparrow$) & Threat \% ($\uparrow$) & Both ($\uparrow$) \\ \hline
WordNet & 12.0 $\pm$ 0.00 & \textbf{18.0 $\pm$ 0.00} & 0.0 $\pm$ 0.00 \\ \hline
Polyjuice & \textbf{55.6 $\pm$ 4.63} & 5.8 $\pm$ 2.6 & 0 $\pm$ 0 \\ \hline
Discover-Adapt (Const 5) & 21.6 $\pm$ 6.05 & 14.0 $\pm$ 5.73& \textbf{2.6 $\pm$ 1.8} \\ \hline
\end{tabular}
\caption{When we treat threat as the held-out dimension, our approach generates more adversarial examples from that dimension. The `Both' metric represents the percentage of generated data point that contain threats as well as adversarial for the classifier. Since the amount of data generated by different methods varies, we report the mean and standard deviation for each method on a sample size of 50 data points bootstrapped for 10 iterations. We only report results of the strongest performing methods of each type.}
\label{tab:obscene-results}
\end{table*}
